Learning from Acceptance: Cumulative Regret in the Game of Coding

Classical coding-theoretic guarantees often rely on trust assumptions, such as requiring sufficiently many honest nodes compared with adversarial ones. These assumptions are difficult to enforce in open decentralized systems where participants are not centrally certified. At the same time, such environments often contain incentive mechanisms: participants may be rewarded only when their submitted data are accepted and the system remains functional. This changes the role of an adversary. Rather than acting as a pure saboteur, a strategic adversary may submit data that are consistent enough to be accepted while still degrading the quality of the final estimate. The game-of-coding framework models this strategic interaction between a data collector (DC) and an adversary. Existing works on the game of coding mostly consider the complete-information case, where the DC knows how the adversary trades off acceptance and estimation error. In this paper, we study an incomplete-information version of the game of coding in which the DC, acting as a Stackelberg leader, does not know the adversary's utility trade-off and must learn through repeated interaction. Prior work on the unknown-adversary setting considered an explore-then-commit objective, where only the final selected acceptance rule is evaluated. In contrast, we study the full learning trajectory: every acceptance rule used during the algorithm is executed and contributes to performance. We propose an algorithm that refines its search around promising acceptance rules, prove that it achieves sublinear cumulative regret, and evaluate its performance through numerical experiments.

==> Figures/Model.tex <==
\begin{figure}[htbp]
    \centering
    \resizebox{0.7\columnwidth}{!}{%
        \begin{tikzpicture}[>=Stealth, thick]

            % Define shapes
            \tikzset{
                block/.style={draw, rectangle, minimum height=10mm, minimum width=22mm, align=center, fill=white},
                diamondblock/.style={draw, diamond, aspect=1.6, minimum width=35mm, minimum height=20mm, align=center, fill=white, inner sep=0pt},
                rejectblock/.style={draw, rounded rectangle, minimum height=10mm, minimum width=22mm, align=center, fill=white}
            }

            % --- ADJUSTED COORDINATES FOR A SMALLER BOX ---
            \def\boxL{0}       % Left edge of Data Collector box
            \def\boxR{9.3}     % Right edge (brought in from 10.5)
            \def\boxT{2.2}     % Top edge (brought down from 3.2)
            \def\boxB{-2.2}    % Bottom edge (brought up from -2.8)
            
            \def\nodeX{-3.8}   % X coordinate for Input Nodes
            \def\nodeY{1.4}    % Y coordinate for Nodes (brought closer vertically)
            
            \def\diaX{3.0}     % X coordinate for Diamond (shifted slightly left)
            
            \def\estX{7.5}     % X coordinate for Estimation block (shifted left)
            \def\rejY{-3}    % Y coordinate for Reject block (moved up)

            % 1. Draw Data Collector background box
            \draw[thick, fill=gray!5] (\boxL, \boxT) rectangle (\boxR, \boxB);
            \node[anchor=south east, font=\large] at (\boxR-0.1, \boxB+0.2) {Data Collector};

            % 2. Draw the Blocks / Nodes
            \node[block] (node1) at (\nodeX, \nodeY) {Node 1};
            \node[block] (node2) at (\nodeX, -\nodeY) {Node 2};
            
            \node[diamondblock] (decision) at (\diaX, 0) {${||\mathbf{Y}_1 - \mathbf{Y}_2||}_2 \leq \eta\Delta$};
            
            \node[block] (estimation) at (\estX, 0) {Estimation};
            
            \node[rejectblock] (reject) at (\diaX, \rejY) {Reject};
            
            \node[font=\Large] (output) at (\boxR + 1.2, 0) {$\hat{\mathbf{U}}$};

            % 3. Draw the connecting arrows
            
            % Node 1 path: Horizontal to the box edge, then diagonal to the diamond
            \draw[->] (node1.east) -- node[above] {$\mathbf{Y}_1 = \mathbf{U} + \mathbf{N}_h$} (\boxL, \nodeY);
            \draw[->] (\boxL, \nodeY) -- (decision.155);
            
            % Node 2 path: Horizontal to the box edge, then diagonal to the diamond
            \draw[->] (node2.east) -- node[above] {$\mathbf{Y}_2 = \mathbf{U} + \mathbf{N}_a$} (\boxL, -\nodeY);
            \draw[->] (\boxL, -\nodeY) -- (decision.205);
            
            % Logic paths
            \draw[->] (decision.east) -- node[above] {Yes} (estimation.west);
            \draw[->] (decision.south) -- node[right] {No} (reject.north);
            
            % Output path
            \draw[->] (estimation.east) -- (output.west);

        \end{tikzpicture}%
    }
  \caption{System model for the $N$-Dimensional game of coding. The network consists of one honest and one adversarial node. Each node reports a noisy version of $\mathbf{U}$ to the DC. For the honest node, the noise $\mathbf{N}_h$ is uniformly distributed within $\mathcal{B}_N( \Delta)$, while for the adversarial node, the noise $\mathbf{N}_a$ follows an arbitrary distribution $g(\cdot)$ chosen by the adversary. Upon receiving the data, the DC decides whether to accept or reject the inputs based on a consistency threshold $\eta$. If accepted, the DC outputs an estimate of $\mathbf{U}$. In this game, the DC acts as the leader choosing $\eta$, and the adversary acts as the follower choosing $g(\cdot)$.}
    \label{fig:Two_node_model}
\end{figure}
